Can Custom Models Learn In-Context? An Exploration of Hybrid Architecture Performance on In-Context Learning Tasks

In-Context Learning (ICL) is a phenomenon where task learning occurs through a prompt sequence without the necessity of parameter updates. ICL in Multi-Headed Attention (MHA) with absolute positional embedding has been the focus of more study than other sequence model varieties. We examine implications of architectural differences between GPT-2 and LLaMa as well as LlaMa and Mamba. We extend work done by Garg et al. (2022) and Park et al. (2024) to GPT-2/LLaMa hybrid and LLaMa/Mamba hybrid models - examining the interplay between sequence transformation blocks and regressive performance in-context. We note that certain architectural changes cause degraded training efficiency/ICL accuracy by converging to suboptimal predictors or converging slower. We also find certain hybrids showing optimistic performance improvements, informing potential future ICL-focused architecture modifications. Additionally, we propose the "ICL regression score", a scalar metric describing a model's whole performance on a specific task. Compute limitations impose restrictions on our architecture-space, training duration, number of training runs, function class complexity, and benchmark complexity. To foster reproducible and extensible research, we provide a typed, modular, and extensible Python package on which we run all experiments.

==> other/lit_review.tex <==


\begin{enumerate}

    % https://arxiv.org/abs/2208.01066
    \todo{figure out how to use bibtex or biblatex lol}
    \item \cite{garg2022can}: What Can Transformers Learn In-Context?
A Case Study of Simple Function Classes (https://github.com/dtsip/in-context-learning)\newline\newline
\hspace*{8 pt} Garg et al showed that Transformers can perform in-context learning. They tested transformers on a variety of function classes: linear functions, sparse linear functions, decision trees and two-layer neural networks. Compared to models like least squares, Lasso, XGBoost, Greedy Tree Learning, 3-Nearest Neighbors and 2-layer NN, they showed that transformers can in-context learn these function classes best or near-best.
\newline\hspace*{8 pt} In addition to the function classes, the paper assessed transformer performance on modified data, specifically on: noisy inputs, limited input domain, and skewed covariance. These tests were only done on linear functions, but indicate that transformers could achieve performance comparable to least squares.\newline

    \item https://arxiv.org/pdf/2111.00396.pdf: Efficiently Modeling Long Sequences with Structured State Spaces (https://github.com/state-spaces/s4)\newline\newline\hspace*{8 pt}
    Gu, Goel, and Re (2022) introduce the structured state space sequence (S4) models as an improvement on state space models and an alternative to other in-context learning models. They show that the S4 model has better speed and memory than transformers, as well as having comparable accuracy with models like LSTMa, Informer, and LogTrans on a variety of metrics. S4 is relevant, given it is a stepping stone to Mamba, which is an architecture of interest.\newline\hspace*{8pt}
    Gu et al also make us of HiPPO matrices to initialize the state space model. Their testing found that HiPPO initialization helps with training and validation accurracy.\newline
    

    \item https://arxiv.org/ftp/arxiv/papers/2312/2312.00752.pdf: Mamba: Linear-Time Sequence Modeling with Selective State Spaces (https://github.com/state-spaces/mamba)\newline\newline\hspace*{8pt}
    Gu and Dao propose Mamba, an improvement on S4 models. Mamba uses a selection mechanism to select data, a hardware-aware algorithm, and a combination of state space model and transformer architectures. Mamba outperforms S4, hence why it is an architecture of interest and was included as an architecture choice.\newline

    \item https://arxiv.org/pdf/2402.04248.pdf: Can Mamba Learn How to Learn?
A Comparative Study on In-Context Learning Tasks (https://github.com/krafton-ai/mambaformer-icl?tab=readme-ov-file)\newline\newline\hspace*{8pt}
    Park et al (2024) evaluate Mamba's ability to perform meta-learning by introducing models to a variety of in-context learning tasks. They find that most state space models can perform in-context learning, but Mamba struggles with decision trees and retrieval tasks while outperforming transformers in other complex tasks.\newline\hspace*{8pt}As a result, they propose the MambaFormer architecture, with the goal of using the advantages of both architectures. Mambaformer is found to be competitive with Transformer and Mamba models, posssessing some advantages such as having the best ICL accuracy among non-LSTM models, though transformers are still superior for language modeling. These observations motivate our interest in hybrid architectures.

    \item https://arxiv.org/pdf/1706.03762.pdf: Attention Is All You Need \newline(https://github.com/tensorflow/tensor2tensor)\newline\newline\hspace*{8pt}
    Vaswani, Shazeer, Parmar, Uszkoreit, Jones, Gomez, Kaiser, and Polosukhin (2023) proposed the transformer architecture, which was a major step forward in in-context learning. The focus on self-attention to do everything allowed for improved parallelization. As a result, the transformer trains quickly compared to architectures dependent on recurrent or convolutional layers while still performing well. This has led transformers to be a baseline that many architectures are compared to today.\newline

    \item https://openreview.net/forum?id=ikwEDva1JZ - "How Do Transformers Learn In-Context Beyond Simple Functions? A Case Study on Learning with Representations." introduces idea of meta functions and combining simple functions\newline\newline\hspace*{8pt}
    Guo, Hu, Mei, Wang, Xiong, Savarese, and Bai (2024) explore transformer performance on compositions fixed representation functions with varying linear functions. While this did appear to impact performance, transformers nevertheless did well, especially with sufficient in-context examples. Their work also showed composition was possibly a simple way to produce more complex function classes.\newline

    \item https://proceedings.neurips.cc/paper\_files/paper/2023/hash/510ad3018bbdc5b6e3b10646e2e35771-Abstract-Conference.html - Exposing attention glitches with flip flop language modeling\newline\newline\hspace*{8pt}
    Liu, Ash, Goel, Krishnamurthy, and Zhang present the "flip-flop" string and a corresponding test - a flip-flop string is a sequence of 0, 1, w, and r. The test is simple - at each r, return the last token after a w. They found that transformers do badly at this simple task, while recurrent models do very well. \newline\hspace*{8pt}This is due to attention, and they present several modifications to attention that alleviate this problem, but none of the solutions are perfect. That said, this paper indicates the necessity of also checking for a model's ability to recall.\newline

    \item https://aclanthology.org/2022.emnlp-main.759/ - Rethinking the role of demonstrations\newline(https://github.com/Alrope123/rethinking-demonstrations)\newline\newline
    \hspace*{8 pt} Min, Lyu, Holtzman, Mikel, Artetxe, Lewsis, Hajishirzi and Zettlemoyer (2022) investigated what knowledge is imparted by in-context learning. They found that when the input data contained randomized labels, rather than the true labels, large language models still performed similarly to the models that were given the true labels. Specifically, performance was similar if the true labels were shuffled around. There was usually a more significant performance decrease if labels were instead random English words. They performed these tests on a wide variety of language models: GPT-2, MetaICL, GPT-J, fairseq, and GPT-3. They also varied the amount of incorrect labels, but found that this did not affect most model accuracy except for GPT-J on classification. \newline\hspace*{8 pt}
    This suggests that in-context learning only teaches language models about the label space and distribution of inputs and outputs. Their findings also suggest that determining whether the truth was learned from the in-context examples may require specialized tests.\newline

    \item https://arxiv.org/pdf/2310.15213.pdf: FUNCTION VECTORS IN LARGE LANGUAGE MODELS (couldn't find a repo)

    \item \cite{wies2024learnability} Wies, Levine, Shashua (2023). The authors give some guarantees on In-Context Learning given some conditions on the pretraining distribution. They also introduce PAC (probably approximately correct) as a measurement of the ability to learn in context learning. PAC means that given $\delta, \epsilon>0$, one cna train the model such that the probability that the loss is greater than $\epsilon$ is less than $\delta$. 

    \item \cite{wei2023larger} Wei et al. The authors find that large language models are able to flip their predictions In-Context if given enough samples of flipped labels, in contrast to smaller models. They are also better at predicting made up category names, suggesting that larger models are able to learn input label mappings in-context, while smaller models often rely on semantic priors. 
\end{enumerate}


==> other/outline.tex <==


% meeting notes
\begin{itemize}
    \item emphasize each training run took very little resources (scaling down. DONE
    \item write about what regression score is and why we think it makes sense as a good proxy. DONE
    \begin{itemize}
        \item discuss context length invariance by design so tasks with very different context lengths can be compared. DONE
        \item also include which optimal predictors are used. DONE
    \end{itemize}
    
    \item regression score is a proxy with which we evaluate a model's ability to ICL. DONE
    \item 
    \item Cite induction heads paper, we don't have enough compute to run our more complex gpt2 configs to the "phase change" for MQAR, thus we have to switch to the Mambaformer paper config so that we can actually see a decrease in loss for MQAR. We also do so to make sure we can compare our results to theirs. DONE
    
    \item finish diagrams for all GPT2 hybrids. DONE
    \item Insert tables. DONE
    \item Ensure table values are correct, fix minor formatting. 
\end{itemize}


\subsection{Results}
\begin{itemize}
    \item Do our results agree with Garg et al. (yes) ... We can then trivially test Llama by leveraging our code design
    
    \item Results of various hybrid arch-es
        \begin{itemize}
            \item we find that more ... shows this qualitative result
        
        \end{itemize}
\end{itemize}

\subsection{Discussion}
\begin{itemize}
    \item our findings with llama suggest ...
        \begin{itemize}
            \item we would  like to recognize that our design with code enabled this to be evaluated easily, as is best illustrated by the subsequent hybrid arch results
            \item because of BLANK, Llama likely did BLANK whereas GPT2 did BLANK
            \item GPT2 achieves similar error to Llama 
        \end{itemize}
    \item our findings with hybrid architectures suggest ...
        \begin{itemize}
            \item we propose the following explanations and defer empirical verification of this hypothesis to future work
        \end{itemize}
    \item Architectural changes to the abstractions in code that occurred as a result of implementing the previous experiments
        \begin{itemize}
            \item To support additional metrics, we had to completely scrap an initial idea for how to process function classes. We were able to keep our abstractions in all other parts of the codebase without needing to rerun training
            \item if any arise in the future, what we did and whether or not the code was able to stay modular 
        \end{itemize}
\end{itemize}

==> other/outline_intro.tex <==
\subsubsection{Intro/ICL as a whole}
\begin{itemize}
    \item What is ICL, transformers are the current object of study wrt this -- Attn All u need \cite{vaswani2017attention}, GPT3 \cite{brown2020language}
    \item ICL is an interesting phenomenon to study -- Many-shot Jailbreaking \cite{anilmany},  \cite{min2022rethinking}, 
    ...?
    % \item However LLMs are prohibitively hard to study in-depth ... (cite gpt4 model card, llama3 paper)
     
    \item "Rethinking the role of demonstrations: What makes in context learning work" introduces interesting ideas about what ICL teaches a model. [discuss paper and resulting tests]
\end{itemize}
%ICL? [discuss beginning of ICL and ICL theory]


\subsubsection{Related benchmark work + function classes}

There have been many techniques for capturing qualitative aspects of ICL with quantitative techniques: 

\begin{itemize}
    \item \cite{weber2023icl} has measured the agreement between a model's predictions in various contexts
    \item Olsson et al 2022 \cite{olsson2022context} compute a heuristic "ICL score" to evaluate the reliance of transformer models on context
    \item Lee et al \cite{lee2023exploring} extend this to other sequence models, including Recurrent and State-space models, finding that although this score reflects some consistencies with other measures, it does not do so universally
    \item Work evaluating ICL often evaluates it through a task for which ICL is the optimal solution \cite{singh2024transient}, \cite{lee2023exploring}, \cite{garg2022can}.
    \item In particular, Garg et al\cite{garg2022can} introduces a scheme for evaluating ICL as a regression or classification task over a handful of simple function classes: ...
    \item Extending this, "Exposing Attention Glitches with Flip Flop Language Modeling" introduces a function class designed to test the models ability to recall information in long context sequences, and compares attention based models to state space models. 
    \item To re-tie the gap from simple function classes to more complex sequence data, "How Do Transformers Learn In-Context Beyond Simple Functions? A Case Study on Learning with Representations" \cite{guo2023transformers} introduces testing on the composition of a fixed representation function and the standard function classes. In their case, they test on Linear regression. 
    % I think this is sufficiently unrelated -- we're interested in architectural effects on ICL ability methinks 
    %\item One such example of one of these more complex sequence modeling tasks is \cite{hsu2022adversarial} "Adverserial Examples Can Be Effective Data Augmentation for Unsupervised Machine Learning". They look at LLMs as general pattern machines, similarly to In-Context learning on simple function classes. They therefore use a set of simple patterns designed for robotics to test the models. These patterns include Probabalistic Context Free Grammar (PCFG), function continuation and physics simulation. They also test token mapping invariance, that is the performance of the model when the tokens in the query are different from what it has seen before, in tasks where the actual tokens are insignificant.
\end{itemize}

\subsubsection{ MHA, MQA, GQA, why ICL happens in attention, SwiGLU+Llama2 stuff}

Olsson et al 2022 \cite{olsson2022context} propose a transformer circuit \cite{elhage2021mathematical} they call an "induction head" they show to likely play a significant role in how transformers perform ICL. 

Min et al 2022 \cite{min2022rethinking} suggest that in-context examples serve as a constraint on an output space (as opposed to a complete evaluation) after which in-weights-learning \cite{singh2024transient} takes over. \cite{singh2024transient} also show that extending training increases this effect.

Todd et al \cite{todd2023function} identify a signature in the residual stream with a causal relationship to transformer predictions 

\subsubsection{MAMBA+SSMs, hybrid architecture discussion}
Analysis of the GPT2-style transformer architecture's in-context learning mechanism has led to interest in whether and how ICL manifests in other sequence models (more specifically, can an attention-less model perform ICL). Chan et. al. (2022) finds that out of a vanilla RNN, LSTM, and traditional tranformer, only the transformer is able to achieve ICL on Zipfian distributions. These results may be attributed to those architecture's limitations in learning that specific task, as Lee et. al. (2024) found that between RNN-style architectures, Transformers (GPT2 and Llama2 style), structured state-space models (SSMs like Mamba, S4, H3), and convolutional neural networks (CNNs), all demonstrated some level of ICL ability but to varying extents and under different conditions. 

Recent ICL research has been doubly motivated to study state-space models due to their low computational complexity. Park et. al. (2024) studies Mamba, S4, and S4-Mamba in depth against transformers and finds that Mamba outperforms transformers in certain tasks like sparse parity, but is outdone in other complex tasks like multi-query associative recall. In a best-of-both-worlds approach, Park et. al. constructs MambaFormer, an architecture possessing Mamba blocks and multi-headed attention. In contrast to Gu \& Dao's (2023) Standard Hybrid, which also combines Mamba and multi-headed attention, MambaFormer replaces positional embeddings with an additional Mamba layer. Both of these hybrid architectures perform comparably to or better than transformer/Mamba on every task. To facilitate further exploration of hybrid architectures, we structure our codebase to allow for easy course and fine-grained architecture customization.

The Standard Hybrid and MambaFormer utilize GPT2 attention in conjunction with Mamba to achieve high ICL performance. How would these architectures perform with different attention styles (e.g. Llama2)? Lee et. al. (2024) demonstrates that Llama2 transformers achieve high multi-class classification and linear regression accuracy on prompt lengths seen in training compared to numerous other architectures, including GPT2-style transformers. Relatively, Llama2 transformers exhibit stronger preferences towards ICL for lower proportions of bursty prompts in their training data distribution, even when Chan et. al. (2022) shows that models achieve "better in-context learning with more burstiness in training." These observations motivate re-exploration of the previously mentioned hybrid architectures with Llama2 instead of GPT2 attention. Thus, a focus of this paper is the analysis of the Llambaformer:

INSERT LLAMBAFORMER DIAGRAM HERE





benchmarks for hybrid: linear regression

\subsubsection{Code ancestry}
There is a wide variety of code styles that work in ICL with simple function classes draws upon:

Direct Descendants of Garg: \cite{ahuja2023closer} \cite{bai2024transformers}

Repos that are too different to say descended: 
\begin{itemize}
    \item \cite{weber2023icl} (because they're not function classes)
    \item \cite{akyurek2024context} (way too comprehensive to have built off of Garg) (these guys might actually just have better code than us, jeez)
\end{itemize}

Else:
\begin{itemize}
    \item \cite{min2022rethinking} older than garg et al -- started with gpt2, later applied to gpt3, solely language
\end{itemize}

    \todo{fill in ancestry graph from lucidspark @nelson}

For the sake of what Donoho \cite{donoho2023data} refers to as Frictionless Reproducibility, we try to model previous software libraries that have made a profound impact in the machine learning community \cite{paszke2019pytorch}, \cite{wolf2020huggingfaces} by providing an extensible codebase with a simple abstraction


==> sections/checklist.tex <==
\section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
%     The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and precede the (optional) supplemental material.  The checklist does NOT count towards the page
%     limit. 
    
%     Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
%     \begin{itemize}
%         \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%         \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%         \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%        % \item {\bf The papers not including the checklist will be desk rejected.}
%     \end{itemize}
    
%     {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.
    
%     The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.
    
%     IMPORTANT, please:
%     \begin{itemize}
%         \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%         \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%         \item {\bf Do not modify the questions and only use the provided macros for your answers}.
%     \end{itemize} 
% %%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The abstract/introduction briefly covers the limitations of the paper while introducing the main claims/findings/contributions. We reference relevant work we are building off of.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We briefly mention some limitations in our analysis and experiments in Section \ref{sec:limitations}. We acknowledge our limited training runs, inexhaustive training horizon, incomplete evaluation of ICL Regression Score, and no metrics on the usability of our codebase. Similarly here we acknowledge that this list of limitations is by no means exhaustive.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: There are no theoretical results or claims in this paper, and thus no assumptions and proofs are required.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss training and evaluation in our paper while making our codebase accessible.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper contributes its codebase, which contains sufficient information in the ReadME for reproducibility. This paper's "Methods" section discusses data generation for the simple function classes. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: These details were explained under the "Methods" section are sufficient to understand our results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Every figure and number presented in this paper has confidence of intervals of 95\% or 99\% (specified in each case).
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The list of all GPU types utilized for the experiments were included, along with the time spent for compute on each of them. Furthermore, we provide a breakdown of the time spent for each experiment type on the GPU that we utilized the most (an A10).
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We study ICL using simple function classes and do not use real world data. No human subjects are involved and there are no direct paths for negative societal impact.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Since this paper studies ICL in hybrid models using simple function classes, there is no direct path to negative applications.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: As this paper discusses ICL on simple function classes, it does not utilize real-world data or models real-world capabilities. Thus, there is no risk for misuse.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide credit to the authors of the three codebases that inspired some of the features in our own and cite that their codebases fall under the MIT License for the first two, and could not be found for the third. URLs are provided for each codebase as well.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our codebase contains a ReadME providing thorough documentation. Our paper also explains high-level functionality of our codebase.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: There are no crowdsourcing experiments or research with human subjects, and thus no text of instructions or compensation information is included.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: As there were no study participants in this study, this information was not included in this paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> sections/limitations.tex <==
We acknowledge that this exploration is incomplete. We have yet to:
\begin{itemize}
    \item Complete all the training runs necessary to reduce the confidence intervals to clearly show that GPT-2 performs notably worse than Llama early in training on Sparse Linear Regression, Linear Regression, and Decision Tree Regression. Currently, these plots are made from only 4 training runs in the sparse linear case and 2 for each of the other two (MLP and DT).

    \item Include our results for Linear Regression between Llama and GPT-2. This is a bit embarrassing as these plots exist but we can't seem to find them. This was a pure miscommunication.

    \item Perform the same style of architectural changes as we proposed for Llama to Mamba between GPT-2 and Llama (i.e. GPT-2 with (1) an RMS Norm pre-norm, (2) with a Llama MLP, (3) with Llama attention (MHA with RoPE), and all combinations of these)
\end{itemize}


==> sections/results_old.tex <==

\subsection{Sparse Linear} As seen in Fig. \ref{fig:comparison-sparse}, the LLaMA and GPT2 models seem to have similar errors at low and high numbers of context examples. As suggested by Garg et al. \cite{garg2022can} and Lee et al. \cite{lee2023attention}, this can be expected by the models estimating the prediction of the optimal predictor. We confirm Lee et al.'s findings that LLaMA is able to learn the optimal predictor. We note that LLaMA appears to be better, especially for five to ten examples, and even for large numbers of in-context examples. However, GPT2 does close the gap as the number of training steps increases, as the difference gradually grows closer to the zero line, and the variance decreases. Still, as can be seen in the actual loss in Figure \ref{fig:loss-sparse}, the difference between LLaMA and GPT2 is relatively small.

\subsection{MLP} %i just wrote something for the sake of having something down for sahai submission, improve on this later
We turn our attention to Fig. \ref{fig:comparison-mlp}. With more training steps, we see a distinct difference between the loss attained by GPT-2 and LLaMA, with GPT2 showing better performance, though LLaMA does have comparative performance when both the number of training steps and in-context examples are low. GPT-2 thus appears to more effectively leverage gradient steps in minimizing loss here. We see that GPT-2's better accuracy over Llama as a function of in-context examples appears to be roughly linear, with the effect becoming more pronounced as the number of training steps increases. Still, as can be seen in the actual loss in Figure \ref{fig:loss-mlp}, the difference is relatively small.

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth,keepaspectratio]{figs/Sparse_diff.png}
        \caption{Sparse Linear Regression}
        \label{fig:comparison-sparse}
    \end{subfigure}
    ~
    \hspace{0.15\textwidth}
    \begin{subfigure}[t]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth,keepaspectratio]{figs/MLP_diff.png}
        \caption{2-layer MLP}
        \label{fig:comparison-mlp}
    \end{subfigure}
    ~ \\
    \begin{subfigure}[t]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth,keepaspectratio]{figs/DT_diff.png}
        \caption{Decision Tree}
        \label{fig:comparison-dt}
    \end{subfigure}
    \caption{The difference in squared error between GPT-2 and Llama regressing onto a parametrized function as a function of in-context examples}
    \label{fig:comparison}
\end{figure}

\subsection{Decision Tree} %i just wrote something for the sake of having something down for sahai submission, improve on this later
We plot these results in Fig. \ref{fig:comparison-dt}. LLaMA outperforms GPT2 quite significantly in this task, and GPT2 only comes close in squared error to LLaMA after many gradient steps (note that in Figure \ref{fig:comparison-dt}, the y-axis shrinks as number of steps increase). This may potentially be explained by the difficulty in learning discrete decision boundaries for the GPT2 architecture, requiring more data than LLaMA to identify the same features. The difference graph appears somewhat similar to that of sparse linear regression, where we see the most improvement over GPT2 towards the middle of the graph. This indicates that at around 100000 steps or more, GPT2 becomes able to catch up to LLaMA with sufficient in-context examples.

That said, the variance in the difference is much wider than that experienced in sparse linear regression. This may indicate that it is possible that either GPT2 or LLaMA has much greater variance when trying to learn decision trees. Indeed, Figure \ref{fig:loss-dt} indicates that it is GPT2 that has much higher variance, and that LLaMA is much more consistent at learning decision trees. Compared to the other tasks, the improvement of LLaMA over GPT2 is also much more significant, especially at fewer training steps.\todo{may need to change once we have linear data}




\begin{figure}
    \centering
    \begin{subfigure}[t]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth,keepaspectratio]{figs/Sparse_pureloss.png}
        \caption{Sparse Linear Regression}
        \label{fig:loss-sparse}
    \end{subfigure}
    ~
    \hspace{0.15\textwidth}
    \begin{subfigure}[t]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth,keepaspectratio]{figs/MLP_pureloss.png}
        \caption{2-layer MLP}
        \label{fig:loss-mlp}
    \end{subfigure}
    ~ \\
    \begin{subfigure}[t]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth,keepaspectratio]{figs/DT_pureloss.png}
        \caption{Decision Tree}
        \label{fig:loss-dt}
    \end{subfigure}
    \caption{The loss GPT-2 and LLaMA regressing onto a parametrized function as a function of in-context examples}
\end{figure}


==> tables/GPU_train_times.tex <==
\begin{figure}[h]
 \centering
    \scalebox{0.8}{
        \begin{tabular}{||cc||}
            \bottomrule \hline
            GPU & Time Trained (hours) \\ 
            \hline \toprule \bottomrule \hline
            A10 & 898.90 \\ 
            RTX 3090 & 55.74 \\
            RTX 4090 & 151.90 \\ 
            RTX 4070 Ti & 75.48 \\
            RTX 6000 & 9.83 \\
            \hline
            Total & 1191.85 \\
            \hline \toprule
        \end{tabular}
    }
    \caption{Time spent training models on each GPU.}
    \label{tab:GPU_train_times}
\end{figure}


==> tables/baselines.tex <==
\begin{table}[ht]
    \centering
    \scalebox{0.8}{
        \begin{tabular}{||c c||}
            \hline
            \toprule
            Task & Baseline Predictor  \\ 
            \midrule
            \hline\hline
            Linear & Least Squares \\ 
            Sparse Linear & LASSO \\
            MLP & 2-layer NN \\ 
            Decision Tree & GPT-2 \\
            Sparse Parity & Mamba \\
            Vector MQAR & Hashmap\\
            \bottomrule
            \hline
        \end{tabular}
    }
    \vspace{0.5em}
    \caption{
        The optimal predictors utilized for each task. The 2-layer NN is trained for 1000 gradient steps, with batches consisting of all of the previous points in the context. GPT-2 is trained for 500k steps on the specified task in the same format as all sequence models of interest.
    }
    \label{tab:baselines}
\end{table}

